Performance Evaluation of ROS2-DDS middleware implementations facilitating Cooperative Driving in Autonomous Vehicle

In the autonomous vehicle and self-driving paradigm, cooperative perception or exchanging sensor information among vehicles over wireless communication has added a new dimension. Generally, an autonomous vehicle is a special type of robot that requires real-time, highly reliable sensor inputs due to functional safety. Autonomous vehicles are equipped with a considerable number of sensors to provide different required sensor data to make the driving decision and share with other surrounding vehicles. The inclusion of Data Distribution Service(DDS) as a communication middleware in ROS2 has proved its potential capability to be a reliable real-time distributed system. DDS comes with a scoping mechanism known as domain. Whenever a ROS2 process is initiated, it creates a DDS participant. It is important to note that there is a limit to the number of participants allowed in a single domain. The efficient handling of numerous in-vehicle sensors and their messages demands the use of multiple ROS2 nodes in a single vehicle. Additionally, in the cooperative perception paradigm, a significant number of ROS2 nodes can be required when a vehicle functions as a single ROS2 node. These ROS2 nodes cannot be part of a single domain due to DDS participant limitation; thus, different domain communication is unavoidable. Moreover, there are different vendor-specific implementations of DDS, and each vendor has their configurations, which is an inevitable communication catalyst between the ROS2 nodes. The communication between vehicles or robots or ROS2 nodes depends directly on the vendor-specific configuration, data type, data size, and the DDS implementation used as middleware; in our study, we evaluate and investigate the limitations, capabilities, and prospects of the different domain communication for various vendor-specific DDS implementations for diverse sensor data type.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
